LoCoML: A Framework for Real-World ML Inference Pipelines

The widespread adoption of machine learning (ML) has brought forth diverse models with varying architectures, and data requirements, introducing new challenges in integrating these systems into real-world applications. Traditional solutions often struggle to manage the complexities of connecting heterogeneous models, especially when dealing with varied technical specifications. These limitations are amplified in large-scale, collaborative projects where stakeholders contribute models with different technical specifications. To address these challenges, we developed LoCoML, a low-code framework designed to simplify the integration of diverse ML models within the context of the \textit{Bhashini Project} - a large-scale initiative aimed at integrating AI-driven language technologies such as automatic speech recognition, machine translation, text-to-speech, and optical character recognition to support seamless communication across more than 20 languages. Initial evaluations show that LoCoML adds only a small amount of computational load, making it efficient and effective for large-scale ML integration. Our practical insights show that a low-code approach can be a practical solution for connecting multiple ML models in a collaborative environment.

==> Sections/introduction_old.tex <==
% Elaborate on how inference is currently done in most systems, and what difficulties arise when manually taking output from one stage and sending it to another, having to write code for every stage etc. Introduce our inference pipeline system which uses models (MDE) and propose it as an alternative to seamlessly perform inference.

The demand for reliable and scalable ML systems is increasing rapidly, with applications in sectors like healthcare, finance, and large-scale industry ~\cite{muccini2021software,lewis2021software}. In these complex environments, ML workflows—such as data preprocessing, model chaining, and inference—pose unique engineering challenges that go beyond those of traditional software systems. As highlighted by Muccini and Vaidhyanathan~\cite{muccini2021software} and Lewis et al.~\cite{lewis2021software}, these challenges become even more significant in scenarios requiring frequent updates, management of data dependencies, and the ability to handle dynamic model behavior, all crucial for maintaining system reliability in real-world production settings.

% Machine Learning (ML) systems are rapidly transforming industries, enabling advancements across diverse sectors through data-driven capabilities. However, managing ML workflows—which includes stages like data preprocessing, model training, and deployment—presents unique software engineering challenges that traditional practices often struggle to address. As ML systems grow, the challenges of handling data dependencies, changing model behavior, and continuous updates become more challenging, all of which are essential for keeping these systems reliable and scalable in production.~\cite{muccini2021software,lewis2021software}.

This work builds on our experience creating a framework to integrate models from diverse sources, each with unique architectures and data needs. Unlike single-model deployments, XYZ project required an inference pipeline capable of handling multiple ML models seamlessly. Meeting this requirement meant designing a multi-model integration framework to overcome compatibility issues common to existing ML workflows, as noted by Amershi et al.~\cite{microsoftSEforML}], who identified multi-model integration and lifecycle management as major gaps in current ML engineering practices.

% Architecting ML-based software systems requires a broader approach to address these challenges. This includes not only structuring and managing ML models but also handling the lifecycle complexities unique to ML components. For example, considerations like data versioning, model compatibility, and cross-functional dependencies create additional demands in ML system engineering~\cite{microsoftSEforML}. The growing need for frameworks that can manage these intricate workflows has highlighted Model-Driven Engineering (MDE)~\cite{schmidt2006model} and Low-Code Development as practical solutions for simplifying and automating various stages of ML pipeline construction. By providing high-level abstractions and visual interfaces, these approaches minimize the need for extensive coding, making ML development more accessible and efficient~\cite{muccini2021software}.

Additionally, the Dagstuhl Seminar on Software Architecture and Machine Learning highlighted key challenges in architecting ML-enabled systems, particularly the integration of ML components into traditional software environments. The seminar highlighted critical architectural attributes such as data-centricity, evolvability, and observability—qualities essential for maintaining reliability in dynamic production settings~\cite{Dagstuhl}. Addressing these attributes requires innovative approaches to manage ML components' lifecycle, including model serving, data transformation, and automated deployment, which traditional software practices often lack~\cite{Dagstuhl}. 

Model Driven Engineering (MDE)~\cite{schmidt2006model} and Low-code development have emerged as practical approaches to simplifying and automating ML pipeline construction~\cite{brambilla2017model}. These frameworks offer high-level abstractions and visual interfaces, as demonstrated by Brambilla, Cabot, and Wimmer~\cite{brambilla2017model}, making complex ML workflows accessible to users with diverse technical backgrounds~\cite{bock2021low}. Low-code platforms, as described by Bock and Frank~\cite{bock2021low}, provide interfaces that connect models and tasks visually, addressing integration challenges ~\cite{di2020democratizing,cabot2020positioning}. 
% These approaches have been proven to enhance efficiency, allowing organizations to manage ML workflows and components across diverse environments
Studies indicate these methods enhance efficiency, enabling organizations to manage ML workflows across varied environments~\cite{appanah2023}. Naveed et al.~\cite{mde4mlslr} emphasis the importance of such platforms, particularly for users who may not have the coding expertise to design or maintain complex ML systems effectively.
Additionally, Low-Code/No-Code platforms have proven effective in democratizing machine learning, as they allow individuals with diverse skill levels to leverage ML models as modular components~\cite{TrinityCollaboration, mlopsCollaboration}. These tools create a shared language, facilitating collaboration among stakeholders with different expertise, and enabling rapid prototyping in a code-free environment, where data scientists, researchers, and domain experts alike can contribute effectively to the AI pipeline creation process.

% Machine Learning (ML) Systems are growing rapidly, with ML models developed for diverse tasks across various fields. However, the process of managing the ML workflows -- such as connecting different stages like data pre-processing, different ML models, and inference -- remains complex. Developers often write code manually for each stage to ensure that output aligns across stages, resulting in time-consuming, error prone workflows that are hard to scale. As ML systems grow in complexity, structured engineering practices are crucial for efficient workflow management, component compatibility, and scalability. 
% Model-Driven Engineering (MDE)~\cite{schmidt2006model} and Low-Code Development can address the limitations of manual coding by automating key aspects of system development and providing high-level abstractions. 

% Brambilla, Cabot, and Wimmer~\cite{brambilla2017model} discuss how MDE practices enhances efficiency and effectiveness in complex software development, which can directly be applicable to ML workflows.

% By adopting proper engineering approaches, like Model-Driven Engineering and Low-code development, we can overcome the limitations of manual coding. This allows for more seamless and efficient ML processes.

% Low-code platforms~\cite{bock2021low} offer a practical solution to these engineering challenges. By providing a visual interface to connect ML models and tasks, they enable pipeline construction with minimal coding~\cite{di2020democratizing,cabot2020positioning}. This approach not only saves time but also makes the ML workflow accessible to people who may have limited coding skills~\cite{appanah2023}. Naveed et al.~\cite{mde4mlslr} highlighted the importance of developing low-code platforms for ML components. They argue that these platforms can significantly reduce the complexity of ML development, especially for non-experts and speed up deployment time. Our framework builds on this foundation. 

To respond to these challenges, we developed LoCoML, a low-code framework designed specifically for building inference pipelines with diverse model types and multi-user roles. LoCoML allows pipeline designers to assemble inference workflows by connecting deployable models and defining logical data flow through a rule-based approach, ensuring compatibility and coherence across stages. Unlike many existing ML workflow solutions, which can face compatibility issues with models from different sources, LoCoML is designed to accommodate various model types, enabling users to chain models seamlessly without extensive manual configuration. This capability is crucial for large-scale AI applications with complex, cross-functional requirements, such as multi-language translation or multi-modal processing.

% In this paper, we introduce LoCoML, a low-code framework focused on simplifying ML inference pipeline development. While LoCoML provides comprehensive support for tasks such as data input, preprocessing, and model training, the scope of this paper is limited to the inference pipeline functionality. This feature allows users to construct inference workflows by connecting deployable models from the repository and configuring logical data flow rules between pipeline stages—all without extensive coding.

For example, in speech-to-text applications, multiple ML models may be needed for tasks like language translation, semantic interpretation, and data processing, with each model having specific preconditions for operation. LoCoML addresses the gap by facilitating model chaining while ensuring quality, compatibility, and system-wide coherence, which are critical in environments where multiple models must work together effectively. Following the AI engineering principles Bosch, Olsson, and Crnkovic~\cite{bosch2021engineering}, LoCoML is built to handle the complexities of multi-model AI pipelines.

% In this paper, we present \textbf{LoCoML}, a low-code framework that enables users to manually add data or use APIs, perform exploratory data analysis (EDA)~\cite{CHATFIELD19865,Komorowski2016}, pre-process data, train models and store deployable models in the repository. These models can be then used in various inference pipelines. However, our focus in this paper is specifically on the inference pipeline aspect. 

\begin{figure}[htbp]
\centerline{\includegraphics[width=\columnwidth]{Figure/LoCoML.png}}
    \caption{Overview of LoCoML Framework}
    \label{fig:locoml_approach}
\end{figure}

The LoCoML framework includes key components, as illustrated in Figure~\ref{fig:locoml_approach}, which provides an overview of the framework. At the core of LoCoML is the ML Flow Orchestrator, which enables pipeline creation and execution by coordinating with other components. The Model Registry stores deployable models, which the Orchestrator accesses to retrieve model details, allowing for seamless integration within inference pipelines. LoCoML also supports different user roles, such as the Pipeline Designer (responsible for creating pipelines), the Pipeline User (who executes the pipelines), and the Model Developer (who trains and registers models). This role-based and grammar-enforced approach ensures that each phase of the ML pipeline lifecycle is handled efficiently, enabling collaboration, flexibility, and logical consistency.

In this paper, we share our experience in developing LoCoML to address the practical needs of organizations and projects requiring robust ML pipeline integration. Through a modular pipeline architecture, LoCoML integrates models from various sources, provides data versioning and model compatibility checks, and enables logical model chaining. Our approach reflects the lessons learned and practical constraints of managing a complex, collaborative ML platform. 

% By adopting a Low-Code Development approach, LoCoML allows users to visually construct pipelines by connecting ML components from preprocessing to inference as modular blocks, while also enabling users to set grammar between blocks to ensure logical and compatible dataflow. This flexibility minimizes complex coding requirements, allowing for rapid ML systems development and deployment and support custom model integration.
% This low-code approach is useful to both technical and non-technical users. 
% It allows them to rapidly develop and deploy ML systems with minimal effort, while also offering the flexibility to integrate custom models.
% Engineering ML systems in this manner not only reduces the barriers for non-experts but also creates more robust, scalable solutions that can adopt to complex requirements. 
% As ML continues to play a major role in various sectors, solutions like LoCoML that combine engineering principles with ease of use will be crucial in making ML development more efficient and accessible.

The remainder of the paper is structured as follows. Section~\ref{sec:motivation} 
% explains the motivation behind our approach, with an example. 
discusses the XYZ project background and it's role as a case study for our approach.
Section~\ref{sec:locoml} describes the LoCoML framework and its core components. Section~\ref{sec:results}, presents the results achieved with the framework. 
% Section~\ref{sec:threats} addresses potential threats to validity. 
A review of related work is in Section~\ref{sec:related_work}, and Section~\ref{sec:conclusion} concludes with summary and future research directions.
